LogicNets: Co-Designed Neural Networks and Circuits for Extreme-Throughput Applications

Deployment of deep neural networks for applications that require very high throughput or extremely low latency is a severe computational challenge, further exacerbated by inefficiencies in mapping the computation to hardware. We present a novel method for designing neural network topologies that directly map to a highly efficient FPGA implementation. By exploiting the equivalence of artificial neurons with quantized inputs/outputs and truth tables, we can train quantized neural networks that can be directly converted to a netlist of truth tables, and subsequently deployed as a highly pipelinable, massively parallel FPGA circuit. However, the neural network topology requires careful consideration since the hardware cost of truth tables grows exponentially with neuron fan-in. To obtain smaller networks where the whole netlist can be placed-and-routed onto a single FPGA, we derive a fan-in driven hardware cost model to guide topology design, and combine high sparsity with low-bit activation quantization to limit the neuron fan-in. We evaluate our approach on two tasks with very high intrinsic throughput requirements in high-energy physics and network intrusion detection. We show that the combination of sparsity and low-bit activation quantization results in high-speed circuits with small logic depth and low LUT cost, demonstrating competitive accuracy with less than 15 ns of inference latency and throughput in the hundreds of millions of inferences per second.

==> content/0-poster.tex <==
\section{Extended Abstract}
Deep Neural Networks (DNNs) have a wide application scope beyond computer vision
tasks, promising to replace manual
algorithmic implementations in applications ranging from large-scale physics
experiments to next-generation network security.
Such applications may require data processing rates in the millions of samples
per second and sub-microsecond latency, which is possible with customized FPGA
or ASIC implementations.
We present a novel method called \OurScheme{} for co-design of DNN
topologies and hardware circuits that maps to a very efficient FPGA
implementation to address the needs of such applications.
% By exploiting the equivalence of artificial neurons with quantized
% inputs/outputs and truth tables, we can
% train sparse, quantized neural networks that can be directly
% and efficiently converted to a netlist of truth tables.
% By carefully controlling the fan-in of the neurons and network topology, we
% can ensure the netlist is small enough to be placed-and-routed onto a single
% FPGA as a highly pipelinable, massively parallel circuit implementing the same
% neural network.

%\section{Method}
% \begin{figure}
% 		\centering
% 		\begin{subfigure}[b]{0.45\textwidth}
% 			\centering
% 			\includegraphics[width=\textwidth]{hbb-neq-redo}
% 			\caption{HBBs and NEQs}
% 			\label{fig:hbbneq}
% 		\end{subfigure}
% 		\par\medskip
% 		\begin{subfigure}[b]{0.45\textwidth}
% 			\centering
% 			\includegraphics[width=\textwidth]{neq-to-hbb-conversion}
% 			\caption{Training and converting a network of NEQs to a netlist}
% 			\label{fig:neqtohbb}
% 		\end{subfigure}
% 		\caption{Summary of the \OurScheme{} design flow.}
% 		\label{fig:schemeoverview}
% \end{figure}

\begin{figure}[!t]
\centering
\subfloat[HBBs and NEQs]{\includegraphics[width=0.45\textwidth]{hbb-neq-redo}%
\label{fig:hbbneq}}
\hfil
\subfloat[Training and converting a network of NEQs to a netlist]{\includegraphics[width=0.45\textwidth]{neq-to-hbb-conversion}%
\label{fig:neqtohbb}}
\caption{Summary of the \OurScheme{} design flow.}
\label{fig:schemeoverview}
\end{figure}

It is possible to convert a neuron with quantized inputs and outputs into a
lookup table (LUT) by evaluating all input-output combinations, as shown in
prior work by Nazemi et al.~\cite{nazemi2018nullanet}.
However, for a neuron with $\gamma$ inputs of $\beta$-bits each, the LUT has
$2^{\gamma \cdot \beta}$ entries and this technique cannot be applied to
most existing DNNs due to dense connectivity and high activation bitwidth.
Instead of mapping existing neural networks to LUTs, we propose to
co-design DNN topologies in a way that avoids intractibly large LUTs.
The key to designing such DNN topologies is to keep the connectivity $\gamma$
and activation bitwidth $\beta$ small.
Figure \ref{fig:schemeoverview} captures the key parts of the \OurScheme{}
approach.
We first define a set of Neuron Equivalents (NEQs) in PyTorch that map to
Hardware Building Blocks (HBBs) generalized as $X$-input $Y$-output LUTs.
Each NEQ is constrained to have a small number of inputs, such that
$X = \gamma \cdot \beta$ maps to at most tens or hundreds of 6:1 FPGA LUTs.
Subsequently, we define and train sparsely-connected neural networks in PyTorch
and convert the trained networks to netlists in Verilog for synthesis,
place and route with Vivado to produce an FPGA bitfile.
By exposing the DNN as a netlist, we are also able to exploit
synthesis optimizations in existing EDA tools to further compress the
DNN to use fewer resources.
%\section{Evaluation}

We evaluate our approach on two tasks with very high intrinsic throughput
requirements.
The first task is the Jet Substructure Classification (JSC) task from
\cite{duarte2018fast}, part of the L1 trigger at the CERN LHC.
The second task is Network Intrusion Detection (NID) by classification of
malicious network packets from \cite{moustafa2015unsw}.
We report out-of-context synthesis results targeting a Xilinx \texttt{xcvu9p-flgb2104-2-i} FPGA.
Our results in Table~\ref{tab:key_results} indicate that the combination of
sparsity and low-bit activation quantization can yield high-speed circuits with
small logic depth, low LUT cost and
competitive accuracy with throughput in the hundreds of millions
of samples per second.

\begin{table}[!t]
\begin{center}
    \caption{Highlights from \OurScheme{} results on the chosen tasks.}
    \label{tab:key_results}
    \begin{tabular}{lllllrr}
    \toprule
    Name & Topology             & $\beta$ & $\gamma$ & Accuracy & LUT    & $F_{\mathrm{max}}$ \\
    \midrule
    JSC-S & 4-layer FC       & 2       & 3        & 84.36\%    & 185    & 1,529~MHz           \\
    JSC-M & 4-layer FC       & 3       & 4        & 87.22\%    & 12,691 & 471~MHz             \\
    JSC-L & 5-layer FC & 3       & 4        & 90.88\%    & 34,740 & 383~MHz             \\
    \midrule
    NID-S & 2-layer FC             & 2       & 7        & 83.88\%    & 3,586  & 811~MHz              \\
    NID-L & 4-layer FC   & 3       & 5        & 88.44\%    & 12,162 & 586~MHz             \\
    NID-M & 4-layer FC   & 2       & 7        & 91.43\%    & 27,129 & 475~MHz             \\
		\midrule
		\multicolumn{7}{l}{\footnotesize \emph{JSC accuracy metric is average area under RoC curve for all classes.}} \\
    \bottomrule
    \end{tabular}
\end{center}
\end{table}


==> content/1-introduction.tex <==
\section{Introduction}
\label{sec:intro}

As the size of Deep Neural Networks (DNNs) continue to grow to improve their
prediction capabilities, their memory and computational footprint also scales
up, making them more and more difficult to deploy on energy and resource
constrained hardware environments.
It has also been shown that DNNs using floating-point arithmetic contain
significant redundancy, which can be exploited  to reduce the compute and
memory cost.
These techniques include quantization, pruning and low-rank decompositions.
Among the proposed techniques for quantization, trained quantization methods
(where the DNN is quantized during the training process) has yielded some of
the most promising results in terms of reducing the workload while maintaining
the accuracy, in the form of Quantized Neural Networks
(QNNs)~\cite{hubara2016quantized}.
The most extreme form of quantization is Binarized Neural
Networks (BNNs)~\cite{courbariaux2016binarized},
where the weights and activations are constrained to binary values, lowering
the compute and memory cost significantly while retaining high accuracy.

In prior work, the strategy for creating an FPGA DNN accelerator, both for QNNs,
BNNs and other DNNs, was to map the artificial neurons to a fixed hardware
architecture by placing the learned parameters in memory and scheduling the
operations so that the correct computations take place between the
corresponding weights and activations.
In turn, the fixed hardware architecture is implemented using LUTs, DSPs and
other FPGA resources.
If we view the problem as a whole, the fixed architecture acts as an interface
between the capabilities of the fabric and the computation that the DNN wants
to do.
However, this interface also acts as a barrier to optimizations that can enable
the DNN to take full advantage of the FPGA fabric.
Furthermore, the fixed architecture requires a non-trivial optimizing compiler
that maps and schedules the DNN computation onto the hardware, which can result
in further performance degradation.

Our method removes the artificial barrier imposed by the fixed hardware
architecture by exposing the building blocks of the FPGA fabric directly to a
machine learning framework.
This approach has the following advantages:

\begin{itemize}
\item Yields extremely efficient DNN accelerators that can classify images
or data at clock rate.
\item No separate hardware architecture or overlay required.
\item No optimizing compiler/scheduler required.
\end{itemize}


==> data/synthopt.tex <==
\pgfplotstableread{
Name	ModelLUT	SynthLUT	LUTsaving
JSC-S	330	185	1.8
JSC-M	42075	12691	3.3
JSC-L	303285	34740	8.7
NID-S	473308	3586	132.0
NID-L	1021175	12162	84.0
NID-M	754292	27129	28.0
}\synthopttable


\begin{tikzpicture}
  \begin{axis}[ybar,bar width=2pt, symbolic x coords={JSC-S, JSC-M, JSC-L, NID-S, NID-L, NID-M}, 
    legend pos=north west, 
    xlabel=Total Neurons,
	ylabel=LUTs,
	ymax = 1200000,
	height=5cm, width=8cm]
    \addplot table[x=Name, y=ModelLUT] {\synthopttable};
    \addplot table[x=Name, y=SynthLUT] {\synthopttable};
    \node at (axis cs:JSC-S,330) [anchor=south]{1.8x};
    \node at (axis cs:JSC-M,42075) [anchor=south]{3.3x};
    \node at (axis cs:JSC-L,303285) [anchor=south]{8.7x};
    \node at (axis cs:NID-S,473308) [anchor=south]{132x};
    \node at (axis cs:NID-L,1021175) [anchor=south]{84x};
    \node at (axis cs:NID-M,754292) [anchor=south]{28x};

    
    \legend{Model LUTs, Post-Synthesis LUTs}
  \end{axis}
\end{tikzpicture}



